Multi-Objective Hyperparameter Tuning and Feature Selection using Filter Ensembles

Both feature selection and hyperparameter tuning are key tasks in machine learning. Hyperparameter tuning is often useful to increase model performance, while feature selection is undertaken to attain sparse models. Sparsity may yield better model interpretability and lower cost of data acquisition, data handling and model inference. While sparsity may have a beneficial or detrimental effect on predictive performance, a small drop in performance may be acceptable in return for a substantial gain in sparseness. We therefore treat feature selection as a multi-objective optimization task. We perform hyperparameter tuning and feature selection simultaneously because the choice of features of a model may influence what hyperparameters perform well. We present, benchmark, and compare two different approaches for multi-objective joint hyperparameter optimization and feature selection: The first uses multi-objective model-based optimization. The second is an evolutionary NSGA-II-based wrapper approach to feature selection which incorporates specialized sampling, mutation and recombination operators. Both methods make use of parameterized filter ensembles. While model-based optimization needs fewer objective evaluations to achieve good performance, it incurs computational overhead compared to the NSGA-II, so the preferred choice depends on the cost of evaluating a model on given data.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = sample-sigconf.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


sample-sigconf.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.thm *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> NOTES <==
## GENERAL 

Submission: https://ssl.linklings.net/conferences/gecco/

* Author Information:
We need to decide who will be present on the conference

* Title: "Multi-Objective Simultaneous Hyperparameter Tuning and Feature Selection using Filter Ensembles" ?

* DONE | Abstract (200 words)

* For final Submission: 

use \citet (textual) and \citep (parenthetical) citation instead of \cite

for anonymous review:
\begin{anonsuppress}
\end{anonsuppress}

'acks' acknowledgements, suppressed in anon mode
\grantsponsor{sponsorid}{name}{url}
\grandnum[url]{sponsorID}{number}

sponsorID can be anything...


## TO-DO's 

* Revise "After the following..." after the rest is done

- Better formulate "Take-Home Messages"
- Immer Bayesian Optimization 
- Check: Define acronyms at their first use.
- remove clean1 dataset, also from table!
- results section
- conclusion
- check captions
- consider mathematical symbols in more places


%% DONE - More Argumentation regarding the overhead of Bayesian Optimization 
%% DONE - All parts that have not been newly introduced/proposed in this study should be presented under the “Background” section.
%% WONTFIX - Cite Andreas Paper and compare to their results
%% DONE - RE-WRITE the abstract and mention Feature Ensembles
%% DONE - describe early stopping xgboost
%% DONE - signifikanzniveau fuer CDT
%% DONE * Was ist citation Guyon-1?
%% DONE - citation LCB: cox1997
%% DONE - What is the representation of each individual? --> kleine Zeichnung  
%% DONE - parameter values that were s.a.
%% DONE - initialization pictures

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Be more clear in describing method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

[Martin]

%% DONE * How did you evaluate each individual on an unseen instance? 
%% DONE - What is the process to measure the fitness function? (see question above)
%% DONE - Following on the previous question, what is the fitness function and what are the objective functions!!? --> Nochmal klarer hinschreiben 
%% DONE - Describe how we initialized the parameter of the geometric distribution; Note that this parameter could be defined by prior knowledge

%%%%%%%%%%%%%%%%%%%%%%%%
%%% Clear up maths
%%%%%%%%%%%%%%%%%%%%%%%%

[Martin]

%% DONE - What erall runtime. Whileis the meaning of m, M and p in Formula (1)?
%% DONE - In individual filter selection, it said that according to filter m. So can I speculate that M represented amount of the filters? But how can you decide it? 
%% DONE - Besides, if m is a filter, so whats [0, 1]^m? 
%% DONE - Shuffling a vector of S 1s and (p - S) 0s makes me confused 
%% DONE - Shorten NSGA2 section, more details about the MBO stuff 

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Clearer argumentation
%%%%%%%%%%%%%%%%%%%%%%%%%%% 

[Both]



%% DONE - "First, the statement should be more concise rather than using too many attributive clause in one sentence", makes the paper hard to understand 
%% DONE - We need to be clearer in that we actually COMPARE our results with SMAC / Bayesian Optimization - an reviewer says that we did not compare, but we actually did

%% DONE - Datasets are quite small, but feature size is high --> emphasize that we consider datasets with a high p / n ratio. 

%% DONE - The direct motivations in the Introduction section are missing. Please discuss the main limitations of the existing methods and highlight how you are planning to address each in this study.
%   - wir sollten erwaehnen:
%     smac kann nicht MO
%     andere machen featsel nicht MO
%     simultaneous wird nur von wenigen gemacht, ist nicht generalisiert (related work wieder reinnehmen)
- NOT RELEVANT %% The title says “Feature Selection”, where is the analysis regarding that part?

%%%%%%%%%%%%%%%%%%%%%%%%
%%% Other things...
%%%%%%%%%%%%%%%%%%%%%%%%

- NOT RELEVANT %% I wonder whether the methods proposed in this paper could be transplanted to it because there are also many hyperparameters in CNN 
- NOT RELEVANT %%  How did you handle the data imbalance issue in your experiments?
- NOT RELEVANT %% How did you deal with the “selection” bias problem?
- DONE %% Shorten the Abstract.
- DONE %% - “This leads in our opinion…post-hoc selection.” Well, this is the core aim of many “multi-objective feature selection” methods. You are not introducing anything new here.
- DONE %% - “It should be noted…under-explored in current ML publications.” Have you checked the literature? There are at least three PhD dissertations have been published dedicated to feature selection/construction.
- DONE %% - It is better to combine the Introduction and Related work and Contributions Section.
- DONE %% - erwaehnen dass unser MBO == smac, nur fuer multi-objective
- DONE %% - Cite Patricks Paper 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Experiments and Results 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

[Julia]

- DONE %% - Forschungsfragen formulieren 
- DONE %% - Suchräume, Filter rein 
- DONE %% - The Evaluation part is very vague. Please improve this part.
- DONE %% Figure 2, lower values are better is confusing (because domHV should be high), but Table 4 and 6 higher values are better. We should formulate that differently! --> we always use higher ranks as better values
- DONE %% - Table 4, no bold results for NSGA-II
- NOT RELEVANT %% - It is probably not necessary to compare over the full objective space, because only a small region might be relevant. --> Adapt analysis here as well
- WONTFIX %% - The experimented methods are stochastic; how many runs have conducted for each method on each dataset? Minimum, 30-50 independent runs should be conducted and the mean and standard deviation should be reported.
- DONE %% - Have you conducted any statistical significance test?
- DONE %% - The parameter settings and justifications are missing.
- DONE %% - what do you mean by “meaningful baseline”?
- DONE %% - warum ist domHV gut? warum waere andere eval willkuerlich?
- DONE %% Random Search goes into the Appendix
- DONE %% - Fuer hypervolume sollten wir Zitzler zitieren (Zitzler & Thiele, 1998).


erall runtime. While
% Filter Ensembles
- Review \citep{Bolon2018} "heterogeneous approach,"
- Comparing Two New Gene Selection Ensemble Approaches with the
Commonly-used Approach:
  - mean aggregation: same as ours, but use dumb mean, we use weights
- Data classification using an ensemble of filters
  - ensemble of pipeline, forward search
- Ensemble Feature Selection: Homogeneous and Heterogeneous Approache
  - different ways of aggregating, among them mean




BO
GA

-MO
-SO

-FE

-NJ

BO-MO-FE-NJ
GA-MO-FE
GA-MO-FE-NJerall runtime. While

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		
